Flat Loss, Evolving Features: Grokking in Modular Addition

Can a network keep learning while its training cross-entropy stays nearly flat at a positive level? We show that it can. On modular addition, a standard testbed for grokking, ReLU networks trained with supported-Polar hidden updates, normalized output-layer updates and weight decay can keep 100% training accuracy while their hidden features change and held-out accuracy rises from zero to above 90%, at relatively flat training cross-entropy. Correct classification need not minimize cross-entropy, which still depends on prediction confidence. We prove this coexistence for one-hidden-layer networks in two finite-window theorems from constructed initializations: one gives a constant gain in the Fourier fraction of the hidden features, and the other holds at arbitrarily low positive loss, where a readout refitted on the training data generalizes before the network. Experiments from random initialization show the same coexistence on a window fixed in advance, and in deeper networks held-out accuracy also rises over post-hoc windows with a net increase in training cross-entropy. With a last-layer rate set per training fraction and head decay scaled with the prime, deeper networks at p=47 and 61 meet a criterion on post-hoc windows, fixed in advance, in nearly all fresh runs. A one-block transformer trained with the same updates and a slowly decaying output gain keeps every training pair correct at every logged checkpoint while its training cross-entropy rises and its held-out accuracy approaches one; with two blocks this holds through the held-out rise, after which training pairs begin to flip. A plateau in training loss need not be a plateau in learning. Code: https://github.com/akashkumar-d/flat-loss-evolving-features.

==> macros.tex <==
\ifdefined\GrokPaperMacrosLoaded\endinput\fi
\def\GrokPaperMacrosLoaded{}
\RequirePackage{amsmath,amssymb,xcolor,etoolbox}

\newif\ifProofRevisionsPending
\ProofRevisionsPendingfalse
\definecolor{proofrevisiongray}{gray}{0.32}
\newenvironment{proofrevision}{%
  \begingroup
  \ifProofRevisionsPending
    \color{proofrevisiongray}\colorlet{eqrefcolor}{proofrevisiongray}%
    \ifdefined\hypersetup
      \hypersetup{linkcolor=proofrevisiongray,citecolor=proofrevisiongray,urlcolor=proofrevisiongray}%
    \fi
  \fi
}{\par\endgroup}
\newcommand{\proofrevtext}[1]{\ifProofRevisionsPending{\color{proofrevisiongray}#1}\else#1\fi}

% Proof-readability changes requested by Akash, 2026-10-14.
% Independent of the orange additions and the historical gray revision switch.
\newif\ifShowReadabilityChanges
\ShowReadabilityChangesfalse
\definecolor{readabilitygreen}{HTML}{17633A}
\newcommand{\readabilitycolor}{%
  \ifShowReadabilityChanges
    \color{readabilitygreen}\colorlet{eqrefcolor}{readabilitygreen}%
    \ifdefined\hypersetup
      \hypersetup{linkcolor=readabilitygreen,citecolor=readabilitygreen,urlcolor=readabilitygreen}%
    \fi
  \fi}
\newrobustcmd{\readability}[1]{{\readabilitycolor#1}}
\newenvironment{readabilityblock}{\begingroup\readabilitycolor}{\endgroup}

% Additions after version 1 (2026-10-13) are printed in dark orange; \ShowAdditionsfalse prints them in black.
\newif\ifShowAdditions
\ShowAdditionsfalse
\definecolor{addedorange}{HTML}{C45100}
\newrobustcmd{\added}[1]{\ifShowAdditions{\color{addedorange}\colorlet{eqrefcolor}{addedorange}%
  \ifdefined\hypersetup\hypersetup{linkcolor=addedorange,citecolor=addedorange,urlcolor=addedorange}\fi#1}\else#1\fi}
\newcommand{\addedcolor}{\ifShowAdditions\color{addedorange}\colorlet{eqrefcolor}{addedorange}%
  \ifdefined\hypersetup\hypersetup{linkcolor=addedorange,citecolor=addedorange,urlcolor=addedorange}\fi\fi}
\newenvironment{additions}{%
  \begingroup
  \ifShowAdditions
    \color{addedorange}\colorlet{eqrefcolor}{addedorange}%
    \ifdefined\hypersetup
      \hypersetup{linkcolor=addedorange,citecolor=addedorange,urlcolor=addedorange}%
    \fi
  \fi
}{\par\endgroup}

\definecolor{notationred}{HTML}{B32222}
\definecolor{notationuses}{HTML}{1756A9}
\definecolor{notationorange}{HTML}{B45A00}
\definecolor{notationgreen}{HTML}{16703A}
\definecolor{notationunclassified}{HTML}{555555}
\newcommand{\notationlabelred}{M}
\newcommand{\notationlabelorange}{A}
\newcommand{\notationlabelgreen}{L}
\newcommand{\notationlabelunclassified}{?}
\newcommand{\notationuse}[4]{%
  \par\smallskip\begingroup\small
  \hypersetup{linkcolor=notationuses}%
  \noindent\textcolor{notation#1}{\textsf{\textbf{[\csname notationlabel#1\endcsname]}}~#2.}\enspace
  \textcolor{notationuses}{Uses: #3.}%
  \ifstrempty{#4}{}{\enspace\textcolor{notationunclassified}{#4}}%
  \par\endgroup\nobreak}

\DeclareMathOperator{\ReLU}{ReLU}
\DeclareMathOperator{\CE}{CE}
\DeclareMathOperator{\Acc}{Acc}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\pol}{pol}
\DeclareMathOperator{\osc}{osc}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\orth}{orth}
\newcommand{\AGOP}{\mathcal G}
\newcommand{\Ginit}{\mathcal G_{\rm init}}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\R}{\mathbb R}\newcommand{\E}{\mathbb E}
\newcommand{\F}{\mathbb F}\newcommand{\one}{\mathbf 1}
\newcommand{\mat}[1]{\boldsymbol{#1}}
\newcommand{\Id}{\mathbb{I}}
\newcommand{\Padd}{\mat{P}_{\mathrm{add}}}\newcommand{\Cgrid}{\mat{C}_{\mathrm{grid}}}
\newcommand{\AH}{A_H}\newcommand{\Train}{\mathcal S}
\newcommand{\Test}{\mathcal D}\newcommand{\Region}{\mathcal R_{p,\Train,M}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\ip}[2]{\left\langle#1,#2\right\rangle}


\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}

\providecommand{\eqdef}{=\mathrel{\mathop:}}
\newtoggle{showcomments}
\settoggle{showcomments}{true}


\iftoggle{showcomments}{
\newcommand{\akash}[1]{{\textcolor{blue}{[{\bf A:} #1]}}}
\newcommand{\sanjoy}[1]{{\textcolor{red}{\rm [{\bf S:} #1]}}}
\newcommand{\annotate}[1]{{\textcolor{blue}{[{\bf Note:} #1]}}}
}
{
\newcommand{\akash}[1]{}
\newcommand{\sanjoy}[1]{}
\newcommand{\annotate}[1]{}
}








\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother
\newcounter{copyrightbox}

\newcommand{\denselist}{
  \itemsep -2pt\topsep-5pt\partopsep-5pt\itemindent-10pt
}
\newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\Rq}{\mathbb{R}^q}
\newcommand{\M}{\mathbb{D}}


\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
\newcommand{\secref}[1]{\textnormal{Section}~\ref{#1}}
\newcommand{\appref}[1]{Appendix \ref{#1}}
\newcommand{\stepref}[1]{Step \ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\conref}[1]{Condition~\ref{#1}}
\newcommand{\assref}[1]{Assumption \ref{#1}}
\newcommand{\remref}[1]{Remark~\ref{#1}}
\newcommand{\egref}[1]{Example~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}


\newcommand{\cf}{\emph{c.f.}}

\newcommand{\op}[1]{\operatorname{#1}}
\newcommand{\paren} [1] {\ensuremath{ \left( {#1} \right) }}
\newcommand{\parenb} [1] {\ensuremath{ \big( {#1} \big) }}
\newcommand{\bigparen} [1] {\ensuremath{ \Big( {#1} \Big) }}
\newcommand{\biggparen} [1] {\ensuremath{ \bigg( {#1} \bigg) }}
\newcommand{\Biggparen} [1] {\ensuremath{ \Bigg( {#1} \Bigg) }}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\tuple}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\newcommand{\curlybracket}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\dist}[2]{\ensuremath{\left\langle#1,\:#2\right\rangle_{\cB}}}
\newcommand{\normg}[2]{\ensuremath{\left\langle#1,\:#2\right\rangle}}
\newcommand{\condcurlybracket}[2]{\ensuremath{\left\{#1\left\lvert\:#2\right.\right\}}}
\newcommand{\inmod}[1]{\ensuremath{\left\lvert\left\lvert#1\right\rvert\right\rvert}}
\newcommand{\boldalpha}{\ensuremath{\boldsymbol{\alpha}}}
\newcommand{\Prover}[2]{\mathop{\textnormal{Pr}}_{#1}\!\,\left[#2\right]}
\newcommand{\cPr}[2]{\ensuremath{\mathop{\textnormal{Pr}}\left\{#1\left\lvert\:#2\right.\right\}}}
\newcommand{\expct}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\expctover}[2]{\mathop{\mathbb{E}}_{#1}\!\left[#2\right]}
\newcommand{\expover}[2]{\mathop{\mathbb{E}}_{#1}\!\Big[#2\Big]}
\def \argmax {\mathop{\rm arg\,max}}
\def \argmin {\mathop{\rm arg\,min}}


\newcommand{\littleO}[1]{\ensuremath{o\paren{#1}}}
\newcommand{\bigO}[1]{\ensuremath{\mathcal{O}\paren{#1}}}
\newcommand{\bigTheta}[1]{\ensuremath{\Theta\paren{#1}}}
\newcommand{\bigOmega}[1]{\ensuremath{\Omega\paren{#1}}}

\newcommand{\bigOTilde}[1]{\ensuremath{\tilde{O}\paren{#1}}}


\newcommand{\NonNegativeReals}{\ensuremath{\mathbb{R}_{\ge 0}}}
\newcommand{\PositiveIntegers}{\ensuremath{\mathbb{Z^+}}}
\newcommand{\integers}{\ensuremath{\mathbb{Z}}}
\newcommand{\nats}{\ensuremath{\mathbb{N}}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\rationals}{\ensuremath{\mathbb{Q}}}
\newcommand{\distrib}[0]{\ensuremath{\mathcal{D}}}
\newcommand{\matroid}{\ensuremath{\mathcal{M}}}
\newcommand{\model}[0]{\ensuremath{\mathcal{M}}}
\newcommand{\sgn}[1]{\operatorname{sgn}\paren{#1}}

\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}

\newcommand{\bL}{{\mathfrak{L}}}
\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bc}{{\mathbf{c}}}
\newcommand{\be}{{\mathbf{e}}}
\newcommand{\bp}{{\mathbf{p}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bZ}{{\mathbf{Z}}}

\newcommand{\rK}{{\mathcal{K}}}

\newcommand{\ff}{{\boldsymbol{\mathfrak{F}}}}
\newcommand{\fr}{{\mathfrak{R}}_{a}}

\newcommand{\col}[1]{\textsf{col}({#1})}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\idot}{\boldsymbol{\cdot}}
\newcommand{\bal}{\boldsymbol{\alpha}}
\newcommand{\cG}{\boldsymbol{\mathcal{G}}}
\newcommand{\bbe}{\boldsymbol{\beta}}
\newcommand{\Hnd}{\boldsymbol{\mathcal{H}}_{n,d}}
\newcommand{\Hndp}{\boldsymbol{\mathcal{H}}_{(n),d}}
\newcommand{\Hndo}{\boldsymbol{\mathcal{H}}_{n-1,d-1}}
\newcommand{\xnd}{\boldsymbol{\mathcal{X}}_{n,d}}
\newcommand{\xndp}{\boldsymbol{\mathcal{X}}_{n,d}^{+}}
\newcommand{\xndn}{\boldsymbol{\mathcal{X}}_{n,d}^{-}}
\newcommand{\Hndd}{\boldsymbol{\mathcal{H}}_{n,d'}^{ind}}
\newcommand{\rnd}{\boldsymbol{\fr}\parenb{\cA(\Hnd)}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\regionset}{\boldsymbol{\mathfrak{R}}\parenb{\mathcal{A}(\Hnd)}}
\newcommand{\regionpair}{\boldsymbol{\mathfrak{R}}\parenb{\mathcal{A}(\boldsymbol{\mathcal{H}}_{(n),d})}}
\newcommand{\lam}{\parenb{\mathbf{\Lambda}}}
\newcommand{\boldlam}{\mathbf{\boldsymbol{\Lambda}}}
\def\mathbi#1{\textbf{\em #1}}
\newcommand{\varstackrel}[3][T]{\stackrel{\raisebox{0.5ex}{\scriptsize#2}}{#3}}
\newcommand{\bg}[1]{g_{#1}}

\def\BState{\State\hskip-\ALG@thistlm}

\newcommand{\data}{\textit{data space}}
\newcommand{\hypo}{\textit{hypothesis space}}
\newcommand{\wrt}{\mathrm{wrt}}
\newcommand{\gen}{{$d'$-\textit{relaxed general position}}}
\newcommand{\up}[1]{\Upsilon_{\mathrm{dual}}\parenb{#1}}
\newcommand{\upi}[1]{\Upsilon^{-1}_{\mathrm{dual}}\parenb{#1}}
\newcommand{\vari}[1]{\varphi^{-1}_{\mathrm{dual}}\parenb{#1}}
\newcommand{\rgn}{r}

\newcommand{\id}[1]{\mathds{1}\left\{#1\right\}}

\newcommand{\sig}{\Sigma_{\mathrm{global}}}


\newcommand{\bestTEQ}{\text{best}-\textnormal{TEQ}}
\newcommand{\randomTEQ}{\text{random}-\textnormal{TEQ}}
\newcommand{\worstTEQ}{\text{worst}-\textnormal{TEQ}}
\newcommand{\binaryTEQ}{\text{binary}-\textnormal{TEQ}}

\newcommand{\maha}{\cM_{\textsf{maha}}}
\newcommand{\tree}{\cM_{\textsf{tree}}}
\newcommand{\graph}{\cM_{\textsf{graph}}}
\newcommand{\fin}{\cM_{\textsf{fin}}}
\newcommand{\nul}[1]{\mathrm{null}({#1})}
\newcommand{\symmp}{\text{Sym}_{+}(\reals^{p\times p})}
\newcommand{\symm}{\text{Sym}(\reals^{p\times p})}
\newcommand{\ranking}[1]{\sigma_{\mathrm{#1}}}
\newcommand{\qfunc}[1]{\ell_{\sigma_{\mathrm{#1}}}}
\newcommand{\qstar}[1]{\ell_{\sigma_{\mathrm{#1}}^*}}
\newcommand{\EQTD}[1]{\text{LwEQ-TD}_{\cX,\cH,h_0}(#1)}
\newcommand{\TD}[1]{\text{LfS-TD}_{\cX,\cH,h_0}(#1)}

\newcommand{\class}[1]{$\cH_{\mathrm{#1}}$}
\newcommand{\lfunc}[1]{$\ell_{\mathrm{#1}}$}
\newcommand{\maxmin}{$\ell_{\mathrm{Max}\text{-}\mathrm{Min}}$}
\newcommand{\hold}{\cH_{\mathrm{threshold}}}


\newcommand{\pp}[1]{[\textbf{\textcolor{red}{PP}: \textsf{#1}}]}

\newcommand{\Binner}[1]{\left(#1\right)}

\newcommand{\MDA}{\textsf{MDA}}
\newcommand{\naive}{\cM_{\sf{NN}}}
\newcommand{\aA}{\mathbcal{A}}
\newcommand{\sA}{\mathrsfso{A}}
\newcommand{\zA}{\mathzapf{A}}
\newcommand{\chA}{\mathchorus{A}}
\newcommand{\sM}{\mathrsfso{M}}

\newcommand{\gm}{\mathchorus{e}}%
\newcommand{\gM}{\mathchorus{E}}%

\newcommand{\sH}{\sf{H}^*_c}
\newcommand{\sHx}{\sf{H}^*_x}
\newcommand{\sMx}{\sf{M}^*_x}
\newcommand{\sHc}[1]{\sf{H}^*_{c(#1)}}
\newcommand{\cd}{\cC}
\newcommand{\re}{\textcolor{purple}{\omega}}
\newcommand{\rer}{\textcolor{black}{\omega}}
\newcommand{\ew}{h(\textcolor{purple}{\omega})}
\newcommand{\ewr}{h(\textcolor{black}{\omega})}
\definecolor{cyanblue}{RGB}{170, 23, 205}
\newcommand{\tcg}[1]{\textcolor{cyanblue}{#1}}
\definecolor{redblue}{RGB}{10, 23, 205}
\newcommand{\tcr}[1]{\textcolor{cyanblue}{#1}}


\newcommand{\ue}{U_{\sf{ext}}}
\newcommand{\g}{\kappa_0}

